Approximate Correlation Clustering Using Same-Cluster Queries

Ashtiani et al. (NIPS 2016) introduced a semi-supervised framework for clustering (SSAC) where a learner is allowed to make same-cluster queries. More specifically, in their model, there is a query oracle that answers queries of the form given any two vertices, do they belong to the same optimal cluster?. Ashtiani et al. showed the usefulness of such a query framework by giving a polynomial time algorithm for the k-means clustering problem where the input dataset satisfies some separation condition. Ailon et al. extended the above work to the approximation setting by giving an efficient (1+\eps)-approximation algorithm for k-means for any small \eps > 0 and any dataset within the SSAC framework. In this work, we extend this line of study to the correlation clustering problem. Correlation clustering is a graph clustering problem where pairwise similarity (or dissimilarity) information is given for every pair of vertices and the objective is to partition the vertices into clusters that minimise the disagreement (or maximises agreement) with the pairwise information given as input. These problems are popularly known as MinDisAgree and MaxAgree problems, and MinDisAgree[k] and MaxAgree[k] are versions of these problems where the number of optimal clusters is at most k. There exist Polynomial Time Approximation Schemes (PTAS) for MinDisAgree[k] and MaxAgree[k] where the approximation guarantee is (1+\eps) for any small \eps and the running time is polynomial in the input parameters but exponential in k and 1/\eps. We obtain an (1+\eps)-approximation algorithm for any small \eps with running time that is polynomial in the input parameters and also in k and 1/\eps. We also give non-trivial upper and lower bounds on the number of same-cluster queries, the lower bound being based on the Exponential Time Hypothesis (ETH).

==> faulty.tex <==
\section{Clustering with Faulty Oracle} \label{sec-faulty} 

In this section we consider the more practical scenario in which the same-cluster query oracle may give wrong answers. More specifically, we assume the answers of the faulty oracle $\OA^E$ to be wrong {\em independently} with probability $0<q\leq \frac{1}{3}$. Given such a faulty oracle, we design query-based polynomial time $(1+\eps)$-approximation algorithms for both $\MA[k]$ and $\MDA[k]$ for any $\eps>0$, and study their query complexities. Our error model is described as follows. We assume that oracle $\OA^E$ pre-computes answers for all possible queries where these query answers may be wrong independently with probability $q$. After pre-computation, every time oracle $\OA^E$ is queried with a pair of vertices $u,v$, it returns $\OA^E(u,v)$ deterministically. Therefore, in our model, success probability can not be amplified by querying the same pair of vertices multiple times. This error model is more relevant in practice because for some pair of vertices, it may not be known with high confidence whether they belong to the same optimal cluster or not.

In Section \ref{sec-upper}, we gave query based $(1+\eps)$-approximation algorithms for $\MA[k]$ and $\MDA[k]$ with a {\em perfect} (no error) query oracle $\OA$. There, given a random sample $S$, we made queries to the oracle $\OA$ to determine how $S$ is partitioned among the $k$ optimal clusters. This partitioning was used crucially in the subsequent analysis. Now, since the oracle $\OA^E$ is faulty, the partitioning method used before would not give exact partitioning of $S$ among the optimal clusters. Instead, we use the algorithm by Mathieu and Schudy in \cite{MS2010} to partition $S$ exactly among optimal clusters with high probability. Mathieu and Schudy studied correlation clustering with noisy input. In their {\em fully-random model} of input, a correlation clustering instance is generated as follows. Starting from an arbitrary base clustering, labels for every pair of vertices are flipped independently with probability $p$ to produce an input instance. Their objective was, given this instance as input, to retrieve the base clustering. The authors showed that if $p\leq \frac{1}{3}$, and the size of every base cluster is $\Omega(\sqrt{n})$ where $n$ denotes the size of vertex set $V$, then their algorithm retrieves the base clustering with high probability. The main result of Mathieu and Schudy that we use in our work is given as follows.

\begin{theorem}[\cite{MS2010}]\label{thm-ms} If $p\leq \frac{1}{3}$, and all base clusters have size $\Omega(\sqrt{n})$, then there is a polynomial time algorithm which retrieves the base clusters exactly with high probability. \end{theorem} 

In this following we give FPTASs for both $\MA[k]$ and $\MDA[k]$ in the SSAC model where the oracle $\OA^E$ may err with some probability $q$. We show, given a random sample $S$, how to construct a correlation clustering instance on $S$ using the query answers as edge labels, and then apply the algorithm of Mathieu and Schudy to retrieve the base clusters with high probability. 

\subsection{$\MA[k]$ with Faulty Oracle} In Section \ref{sec-upper}, we gave a query based FPTAS for $\MA[k]$ in the SSAC model with a perfect oracle $\OA$. Here we show how to modify that algorithm to make it work with a faulty oracle $\OA^E$. The modified algorithm is given as Algorithm \ref{alg-fma}. Let $V^1,\ldots,V^m$ be a random partition of $V$ for $m=O(\frac{1}{\eps})$ such that $|V^1|=\ldots=|V^m|$. The algorithm works in $m$ iterations where in $i$th iteration $V^i\subseteq V$ is clustered using a random sample $S^i$ from $V\setminus V^i$. In Algorithm \ref{alg-ma}, oracle $\OA$ was used to partition random sample $S^i$ in the $i$th iteration such that the partition $S^i=S^i_1 \cup \ldots \cup S^i_k$ satisfies $S^i_j=S^i\cap D_j$ where $D=\{D_1,\ldots,D_k\}$ is the optimal clustering. To partition $S^i$ as above with a faulty oracle $\OA^E$, we first query oracle $\OA^E$ with all pairs of vertices in $S^i$. Using these query answers, an instance of correlation clustering is constructed on $S^i$ where label for any edge $(u,v)$ is $\OA^E(u,v)$. Note that the correlation clustering instance, generated as above, can be thought of being generated in the {\em fully-random} input model of Mathieu and Schudy. The base clustering in this setting would correspond to the partitioning of $S^i$ as in the optimal clustering. We use the algorithm of Mathieu and Schudy to retrieve the base clustering of $S^i$ with high probability in $i$th iteration of our algorithm for $1\leq i\leq m$. The following lemma shows that the correlation clustering instance generated above satisfies the condition that $|S^i_j|\geq \sqrt{|S^i|}$ for all $1 \leq j \leq k$ for Theorem \ref{thm-ms} to hold. Also, since $S^i$s are not independent, we show the overlap of $S^i$ and $S^j$ for any $i\neq j$ is not much.

The following lemma shows that for a random sample $S^i$ to have all its optimal partitions $S^i_j$ of large size, all the optimal clusters of the graph $G$ have to be large.
\begin{lemma}\label{lemma-fma-1} Let us assume that all optimal clusters are of size at least $n^{3/4}$. Then, for random sample $S^i$ of size $|S^i|=O(\frac{\sqrt{n}}{k\eps^2}\log \frac{m}{\eps \delta})$, we have $|S^i_j|\geq \sqrt{|S^i|}$ for $1\leq j\leq k$ whp.\end{lemma}
\begin{proof} Let $D_1,\ldots,D_k$ be the optimal clusters of $G(V,E)$ such that $|D_j|\geq n^{3/4}$ for $1\leq j\leq k$. For any $j$ and any $u\in D_j$, the probability that $u$ belongs to sample $S^i$ is $\frac{|S^i|}{n}$. Therefore, $\EE[|S^i_j|]=\EE[|S^i\cap D_j|]=O(\frac{n^{1/4}}{k\eps^2}\log \frac{m}{\eps \delta}) \geq \sqrt{|S^i|}$. Using Chernoff bounds, for some constant $0<\gamma<1$, with probability at least $1-k e^{-O(n^{1/4})\frac{\gamma^2}{2}}$, $|S^i_j|\geq \sqrt{|S^i|}$ holds for $1\leq j\leq k$.
\end{proof}

In the following we prove that the overlap between any two random samples is not large. Let the size of random samples for any iteration $i$ be $|S^i|=O(\frac{\sqrt{n}}{k\eps^2}\log \frac{m}{\eps \delta})$.

\begin{lemma}\label{lemma-fma-2} There is at most a constant overlap between any pair of random samples $S^i$ and $S^j$ with $i\neq j$ with high probability.\end{lemma}
\begin{proof} Let $X_u$ denote a random variable such that $X_u=1$ if $u\in S^i\cap S^j$ for some $i\neq j$, and $0$ otherwise. Then expected overlap between $S^i$ and $S^j$ is $\EE[S^i\cap S^j]=\sum_{u\in V} \Pr[u \in S^i\cap S^j]=\frac{|S^i||S^j|}{n}=O(\frac{\log^2 \frac{m}{\eps \delta}}{k^2 \eps^4})$, a constant. Using Markov's inequality, $\Pr[|S^i\cap S^j|> O(\frac{16\log^2 \frac{m}{\eps \delta}}{k^2 \eps^6})] \leq \frac{\eps^2}{16 k^2}$. Since $m=\frac{4}{\eps}$, the probability that for all $S^i$ and $S^j$ with $i\neq j$, there is at most constant overlap between $S^i$ and $S^j$ is at most $\frac{1}{k^2}$. \end{proof}


In the subsequent discussion and for the results we derive next, we assume that the above two conditions hold. The query based FPTAS for $\MA$ with oracle $\OA^E$ is given as Algorithm \ref{alg-fma}. This algorithm is almost the same as query based FPTAS Algorithm \ref{alg-ma} for $\MA$ with oracle $\OA$. We highlight the differences here. In Step $1$ of Algorithm \ref{alg-fma}, we consider a random partition of $V$ into $V^1,\ldots,V^m$ whereas we considered any arbitrary partition of $V$ in Algorithm \ref{alg-ma}. Also, the size of the random sample $S^i$ in $i$th iteration would be substantially larger in Algorithm \ref{alg-fma} than in Algorithm \ref{alg-ma}.

From Lemma \ref{lemma-fma-1}, we have for random sample $S^i$ in iteration $i$, all of its optimal partitions $|S^i_j|$ are of size at least $\Omega(\sqrt{S^i})$ for all $j$. Lemma \ref{lemma-fma-2} ensures that there is not much overlap between any two random samples. For error probability $q\leq \frac{1}{3}$, the algorithm by Mathieu and Schudy retrieves the base clustering $S^i=\{S^i_1,\ldots,S^i_k\}$ with high probability. Once $S^i$ is partitioned as in the optimal clustering, following similar reasoning as in Algorithm \ref{alg-ma}, the query Algorithm \ref{alg-fma} would give $(1+\eps)$-approximation for $\MA[k]$. Since we query the oracle with all pairs of vertices in $S^i$, $i$th iteration uses at most $|S^i|^2$ same-cluster queries. Since the algorithm works in $O(\frac{1}{\eps})$ iterations, the total number of queries used by the algorithm is $O({\frac{1}{\eps}} {|S^i|^2})$. When $|S^i|=O(\frac{\sqrt{n}}{k\eps^2} \log \frac{m}{\eps \delta})$, the number of queries is $O(\frac{n}{k^2 \eps^5} \log^2 \frac{m}{\eps \delta})$. Our main result for $\MA[k]$ is given as follows. 

\begin{center}
\begin{Algorithm}
\begin{boxedminipage}{\textwidth}
$\mathsf{FaultyQueryMaxAgree(k,\eps)}$

\underline{Input}: Labeling $\mathcal{L}:{n\choose 2} \rightarrow \{+,-\}$ of edges of graph $G(V,E)$, Oracle $\OA^E:{n\choose 2}\rightarrow \{\text{Yes,No}\}$.\\
\underline{Output}: A $k$-clustering of $G$\\ \\
\hspace*{0.0in}(1) Construct a random partition of the graph into roughly equal parts $(V^1,\ldots,V^m)$ where $m=\lceil \frac{4}{\eps} \rceil$.\\
\hspace*{0.0in}(2) For $i=1,\ldots,m$, choose uniformly at random with replacement from $V\setminus V^i$, a subset $S^i$ of size $r=O(\frac{\sqrt{n}}{k\eps^2}\log \frac{m}{\eps \delta})$.\\
\hspace*{0.0in}(3) Set $W$ to be an arbitrary clustering.\\
\hspace*{0.0in}(4) {\bf Cluster $S^i=\{S^i_1,\ldots,S^i_k\}$ by making same-cluster queries to oracle $\OA^E$.}\\
\hspace*{0.2in}(a) $\forall i=1,\ldots,m$: do the following.\\
\hspace*{0.3in}(i) For each vertex $v\in V^i$ do.\\
\hspace*{0.4in}(1) For $j=1,\ldots,k$ let\\
\hspace*{0.5in}$\beta_j(v)=|\Gamma^{+}(v)\cap S^i_j|+ \Sigma_{l\neq j} |\Gamma^{-}(v)\cap S^i_l|$ where $\Gamma^{+}(v)$ and $\Gamma^{-}(v)$ are the sets of vertices adjacent to $v$ with a $`+'$ or $`-'$ edge respectively.\\
\hspace*{0.4in}(2) Place $v$ in cluster $arg\max_j \beta_j(v)$.\\
\hspace*{0.2in}(b) If the clustering formed in step (a) has more agreements than $W$, set $W$ to be that clustering.\\
\hspace*{0.0in}(5) Output $W$.\\
\end{boxedminipage}
\caption{Faulty Query version of the $\MA$ algorithm by Giotis and Guruswami.}
\label{alg-fma}
\end{Algorithm}
\end{center}


\begin{theorem} There is a query algorithm $\mathsf{FaultyQueryMaxAg}$ that behaves as follows: On input $\veps,\delta$ and a labelling $\mathcal{L}$ of the edges of a complete graph $G$ with $n$ vertices with each optimal cluster of size at least $n^{3/4}$, with probability at least $(1-\delta)$, algorithm $\mathsf{FaultyQueryMaxAg}$ outputs a $k$ clustering of the graph such that the number of agreements induced by this $k$-clustering is at least $OPT-\veps n^2/2$, where $OPT$ is the optimal number of agreements induced by any $k$-clustering of $G$, where oracle $\OA^E$ errs with probability $q\leq \frac{1}{3}$. The running time of the algorithm is $O(n~ \text{poly}(k,\frac{1}{\eps}))$. Moreover, the number of same-cluster queries made by $\mathsf{FaultyQueryMaxAg}$ is $O \left( \frac{n}{k^2\veps^5} \log^2{\frac{m}{\veps \delta}}\right)$. \end{theorem}

Using the observation that $OPT\geq n^2/16$ (see proof of Theorem 3 in \cite{GG2006}), we obtain the above query algorithm is an FPTAS in the SSAC framework with faulty oracle.




\subsection{$\MDA[k]$ with Faulty Oracle} In Section \ref{sec-upper}, we obtained a query based FPTAS for $\MDA[k]$ in the SSAC model with oracle $\OA$. Now we show how to modify that algorithm to make it work with the faulty oracle $\OA^E$. In the query based algorithm (Algorithm \ref{alg1}), to partition random sample $S$ among optimal clusters, we made same-cluster queries to the oracle $\OA$ to obtain $k$-partitioning of $S=S_1 \cup \ldots \cup S_k$ such that $S_i=S\cap D_i$ where $D_1,\ldots,D_k$ are the optimal clusters. Now, with faulty oracle $\OA^E$, in order to partition $S$ as in the optimal clustering, we apply the algorithm by Mathieu and Schudy \cite{MS2010}. As in the previous section, in order to ensure that the optimal partitions of random sample $S$ are of large size, we need all the optimal clusters of the graph to be large. From Lemma \ref{lemma-fma-1}, assuming all optimal clusters are of size at least $n^{3/4}$, we get that for any random sample $S$ of size $O(\frac{\sqrt{n}}{k\eps^2}\log \frac{m}{\eps \delta})$, clusters $S_j=S\cap D_j$ have size at least $\sqrt{|S|}$ with high probability. The following lemma shows that with high probability there is only constant overlap between any pair of random samples.

\begin{lemma}\label{lemma-fmda-1} There is only constant overlap between any pair of random samples with high probability. \end{lemma}
\begin{proof} The proof of this lemma is similar to the proof of Lemma \ref{lemma-fma-2}. There we observed that for any two distinct random samples $S^i$ and $S^j$, with probability at least $1-\frac{\eps^2}{16k^2}$, the overlap between $S^i$ and $S^j$ is at most $O(\frac{16\log^2 \frac{m}{\eps \delta}}{k^2 \eps^6})$. Since there can be at most $k$ different random samples in this case, with probability at least $1-\frac{\eps^2}{16}$, the overlap between any two random samples is at most $O(\frac{16\log^2 \frac{m}{\eps \delta}}{k^2 \eps^6})$. \end{proof}

In the subsequent discussion we assume that all optimal clusters are large and any two random samples have only constant overlap with high probability. Our results are derived assuming the above to be true. Given a random sample $S$, we query the oracle $\OA^E$ with all pairs of vertices in $S$ to construct an instance of correlation clustering. This instance is then fed to the algorithm of Mathieu and Schudy to retrieve base partitioning of $S$ among optimal clusters with high probability. Since we query the oracle for all pairs of vertices in $S$, the number of queries in one iteration is at most $|S|^2$. The analysis of the algorithm remains the same as in for Algorithm \ref{alg1} with the exception that the number of queries varies. For $|S|=O(\frac{\sqrt{n}}{k\eps^2}\log \frac{m}{\eps \delta})$, we have the number of queries in one iteration to be $O(\frac{n}{k^2\eps^4}\log^2 \frac{m}{\eps \delta})$. Combining this number with the number of queries used in $\mathsf{FaultyQueryMaxAg}$, the total number of queries used in one iteration is $O(\frac{nk^{18}}{\eps^{10}})$. We have the main result of the section as follows.

\begin{theorem} Let $0<\veps\leq 1/2$. For any input labelling of graph $G(V,E)$, and assuming all optimal clusters are of size at least $n^{3/4}$, $\mathsf{FaultyQueryMinDisAgree(k,\veps/4)}$ returns a $k$-clustering with the number of disagreements within a factor of $(1+\veps)$ of the optimal with high probability using only $O(\frac{nk^{19}}{\eps^{10}})$ same-cluster queries and running in $O(n\log n~\text{poly}(k,\frac{1}{\eps}))$ time where oracle errs with probability $q\leq \frac{1}{3}$.\end{theorem}


==> notes.tex <==
\section*{Notes for Myself} 
\begin{itemize}
	\item {[Date: 18/09/2017]} I wrote to the authors of Fomin \etal~to check if they know of any such result. Pilipczuk replied saying that even if there exists such a reduction, it is not direct, and he does not see any easy modification for such a result. Moreover, he gave intuition about why obtaining such a result may be non-trivial. Overall he is not sure. I spoke with Ragesh about sending the manuscript to LATIN without much changes, and he kind of agreed.
	\item {[Date: 15/09/2017]} The challenge in lower bound is to check whether the reduction of Fomin \etal~is or is not approximation preserving. If it is an approximation preserving reduction, then what kind of lower bounds can one obtain for this problem? To show approximation preserving reduction, do the following. More precisely, given a $3$-SAT instance $\phi$, if there exists a satisfying assignment for $\phi$ show that the reduced instance has cost at most $k^{\prime}>k$, where $k$ is the number of optimal clusters. This part along with the other direction is shown by Fomin \etal. We need to show that for some $\eps>0$, if no assignment satisfies more than $(1-\eps)$-fraction of clauses of $\phi$, then the cost of the reduced instance is at least $k^{\prime}(1+\eps^{\prime})$ for some $\eps^{\prime}>0$.
\end{itemize}

